Active Neural Matter: A Finite-Window Response Framework for Physical Systems and Distributed AI Workflows

Physical systems and distributed AI workflows can retain past information, receive delayed feedback and combine conflicting signals. These features pose a common modeling problem: determining what information about past interactions a state must retain to account for future responses. Active Neural Matter (ANM) addresses this problem through a finite-window response framework. Forward analysis uses each system's dynamics to predict state and output responses to perturbations, separating propagation from output sensitivity. Inverse analysis tests whether a candidate state retains enough information for these responses. With the system and future inputs or interaction rules fixed, distinguishable responses from histories assigned the same state identify distinctions the representation must preserve. Their distributional separation gives a lower bound on the worst-case error of approximating behavior from that state. Uncertainty bounds distinguish rejection, support within a fixed tolerance on tested comparisons, and unresolved cases. Delayed-consensus simulations check analytical predictions of response amplitude and phase over a narrow range of delays; flocking illustrates dependence on the chosen observable. An exact delayed-return construction establishes a sufficient state for a specified program. The AI studies identify distinctions in interaction history and evidence order that a representation must preserve to reproduce observed response distributions. Tests on new histories in a controlled feedback task provide bounded support for a state specified by the task instructions; the instructed rule predicts every observed action. ANM connects response prediction to measurable information requirements, separating behavioral fidelity from task correctness and initial-state adequacy from a closed evolution law for that state.

==> references_to_main.tex <==
% Generated cross-document reference numbers; verified by the release build.
\expandafter\def\csname publicref@eq:adaptive-workflow\endcsname{1}
\expandafter\def\csname publicref@eq:ai-candidate-readout\endcsname{21}
\expandafter\def\csname publicref@eq:ai-graph-update\endcsname{19}
\expandafter\def\csname publicref@eq:ai-paired-measurement\endcsname{22}
\expandafter\def\csname publicref@eq:ai-reader-input\endcsname{20}
\expandafter\def\csname publicref@eq:anm-universal-interface\endcsname{6}
\expandafter\def\csname publicref@eq:compression-diameter\endcsname{32}
\expandafter\def\csname publicref@eq:consensus-harmonic-susceptibility\endcsname{12}
\expandafter\def\csname publicref@eq:consensus-harmonic-targets\endcsname{14}
\expandafter\def\csname publicref@eq:consensus-operating-criteria\endcsname{15}
\expandafter\def\csname publicref@eq:consensus-window-readout\endcsname{13}
\expandafter\def\csname publicref@eq:finite-graph-linear-response\endcsname{2}
\expandafter\def\csname publicref@eq:finite-window-endpoint-response\endcsname{3}
\expandafter\def\csname publicref@eq:flock-averaged-readouts\endcsname{18}
\expandafter\def\csname publicref@eq:flock-instantaneous-readouts\endcsname{17}
\expandafter\def\csname publicref@eq:public-consumer-equivalence\endcsname{27}
\expandafter\def\csname publicref@eq:public-local-source\endcsname{7}
\expandafter\def\csname publicref@eq:public-matching-bound\endcsname{5}
\expandafter\def\csname publicref@eq:public-representation-transfer\endcsname{29}
\expandafter\def\csname publicref@eq:public-state-discrepancy\endcsname{28}
\expandafter\def\csname publicref@eq:public-stationary-susceptibility\endcsname{8}
\expandafter\def\csname publicref@eq:supp-consensus-mean-eq\endcsname{11}
\expandafter\def\csname publicref@eq:supp-driven-consensus\endcsname{10}
\expandafter\def\csname publicref@eq:vicsek-field\endcsname{16}
\expandafter\def\csname publicref@fig:closed-loop\endcsname{6}
\expandafter\def\csname publicref@fig:inverse-validation\endcsname{5}
\expandafter\def\csname publicref@fig:mechanism-controls\endcsname{2}
\expandafter\def\csname publicref@fig:physical-realizations\endcsname{4}
\expandafter\def\csname publicref@fig:reduced-frontier\endcsname{3}
\expandafter\def\csname publicref@fig:scientific-evidence\endcsname{7}
\expandafter\def\csname publicref@fig:universal-pipeline\endcsname{1}
\expandafter\def\csname publicref@iclr:ai-evidence\endcsname{4}
\expandafter\def\csname publicref@iclr:ai-statement\endcsname{11}
\expandafter\def\csname publicref@iclr:conditions\endcsname{3.3}
\expandafter\def\csname publicref@iclr:discussion\endcsname{10}
\expandafter\def\csname publicref@iclr:eq-kernel\endcsname{4}
\expandafter\def\csname publicref@iclr:eq-nested\endcsname{9}
\expandafter\def\csname publicref@iclr:introduction\endcsname{1}
\expandafter\def\csname publicref@iclr:main-end\endcsname{11}
\expandafter\def\csname publicref@iclr:physics\endcsname{3}
\expandafter\def\csname publicref@iclr:pre-references-end\endcsname{11}
\expandafter\def\csname publicref@iclr:protocol\endcsname{2}
\expandafter\def\csname publicref@iclr:references-start\endcsname{11}
\expandafter\def\csname publicref@iclr:reproducibility\endcsname{11}
\expandafter\def\csname publicref@sec:adaptive-response\endcsname{2.1}
\expandafter\def\csname publicref@sec:closed-loop\endcsname{6}
\expandafter\def\csname publicref@sec:compression-error\endcsname{8.3}
\expandafter\def\csname publicref@sec:cross-domain\endcsname{2}
\expandafter\def\csname publicref@sec:crossed-routing\endcsname{5.4}
\expandafter\def\csname publicref@sec:information-requirements\endcsname{8}
\expandafter\def\csname publicref@sec:public-methods\endcsname{11}
\expandafter\def\csname publicref@sec:routing-refinement\endcsname{5.5}
\expandafter\def\csname publicref@sec:routing-sufficiency\endcsname{5.2}
\expandafter\def\csname publicref@sec:scientific-evidence\endcsname{7}
\expandafter\def\csname publicref@sec:worked-tool\endcsname{5}
\expandafter\def\csname publicref@si:consumer-family\endcsname{8.1}
\expandafter\def\csname publicref@si:eq-inverse-continuation\endcsname{24}
\expandafter\def\csname publicref@si:eq-inverse-readout\endcsname{23}
\expandafter\def\csname publicref@si:eq-model-tv-lower\endcsname{26}
\expandafter\def\csname publicref@si:eq-model-tv-upper\endcsname{25}
\expandafter\def\csname publicref@si:inverse-model\endcsname{5.3}
\expandafter\def\csname publicref@si:inverse-mwe\endcsname{5.1}
\expandafter\def\csname publicref@si:nested-observables\endcsname{3.3}
\expandafter\def\csname publicref@si:observables-directions\endcsname{3.3}
\expandafter\def\csname publicref@si:related-work\endcsname{9}
\expandafter\def\csname publicref@si:tab-inverse-mwe\endcsname{4}
\expandafter\def\csname publicref@si:worked-graph\endcsname{4}
\expandafter\def\csname publicref@tab:cross-domain-roles\endcsname{1}
\expandafter\def\csname publicref@tab:phys-anm-compact\endcsname{3}
\expandafter\def\csname publicref@tab:response-judgments\endcsname{2}

